Boosting 5G mm-Wave IAB Reliability with Reconfigurable Intelligent Surfaces

The introduction of the mm-Wave spectrum into 5G NR promises to bring about unprecedented data throughput to future mobile wireless networks but comes with several challenges. Network densification has been proposed as a viable solution to increase RAN resilience, and the newly introduced Integrated-Access-and-Backhaul (IAB) is considered a key enabling technology with compelling cost-reducing opportunities for such dense deployments. Reconfigurable Intelligent Surfaces (RIS) have recently gained extreme popularity as they can create Smart Radio Environments by EM wave manipulation and behave as inexpensive passive relays. However, it is not yet clear what role this technology can play in a large RAN deployment. With the scope of filling this gap, we study the blockage resilience of realistic mm-Wave RAN deployments that use IAB and RIS. The RAN layouts have been optimised by means of a novel mm-Wave planning tool based on MILP formulation. Numerical results show how adding RISs to IAB deployments can provide high blockage resistance levels while significantly reducing the overall network planning cost.

==> content/3_base_model.tex <==
\color{red}TODO EUGENIO\color{black}\newline
%In this section we describe the dual homing coverage planning formulation with IAB.\newline
In this section, we describe a coverage planning formulation where the blockage-resilience of a mm-Wave IAB access network is boosted by means of reconfigurable intelligent surfaces.\newline
Indeed RIS are installed and configured such that they provide an alternative radio path between the transmitting IAB node and the receiving UE, should the direct line of sight be interrupted by an obstacle. Other planning works have shown how this approach is effective in
Similarly to what has been done in other coverage planning works~\cite{AMALDI20082159,devoti2020},
we consider a set $\C$ of Candidate Sites (CSs) over a geographic area covered by a mm-wave access service. Each candidate site represents the position where a BS can be installed, namely a donor or an IAB node. A set of Test Points (TPs) $\T$ represents the user distribution over the same area.\par
We have considered dual homing in this work. That is, we allow each TP to be associated with a primary BS and a backup BS.\newline
The rationale behind this approach is to provide each TP with a backup link that ensures the continuity of connectivity when the primary link is obstructed.\newline
However, a single but large obstacle could interrupt TP's primary and backup links if these present low angular separation, leading to a connection outage and decreasing the efficacy of dual homing. As such, our model favours the activation of those backup and primary links with higher angular separation. This is achieved by considering parameter $\Theta_{t,c,d}$, that denotes the smallest angle between CSs $c$ and $d$, as seen from TP $t$.\newline
Link length represents another factor influencing the network resilience to blockages. Indeed, longer radio connections naturally experience higher probabilities of being blocked by one or more obstacles~\cite{Akdeniz2014}. In our formulation, we favour the activation of shorter access links, such that each one is individually less inclined to be blocked. Parameter $L_{t,c}$ represents the distance between TP $t$ and CS $c$.\par
Physical parameters and propagation characteristics, such as transmit power, receiver sensitivity and attenuation losses are captured by a binary activation link parameter $\Lambda{t,c,d}$. This is 1 only when a radio connection can be established between TP $t \in \T$, primary BS in CS $c \in \C$ and backup BS in CS $d \in \C$. Moreover, fixed obstacles across the geographic area interrupting any line of sight can be modeled by setting the corresponding link activation parameter to 0.\newline
Similarly, binary parameter $\Delta{c,d}$ indicates whether two BSs in CSs $c,d\in \C$ can establish a radio backhaul link.\par
Given the fixed positions of TPs and CSs, achievable downlink rates in backhaul and access can be computed according to transmitter-receiver characteristics and any propagation model of choice. The extreme directivity of mm-Wave downlink transmissions limits the interference effects and we assume these achievable rates to be unaffected by simultaneous transmissions\cite{devoti2020}.\newline
In our formulation, the achievable downlink rate between a generic TP $t$ and BS installed in CS $c$ is expressed through parameter $V_{t,c}$. In a similar fashion, the capacity of a backhaul link established between two BSs $c$ and $d$ is denoted by parameter $U_{c,d}$.\par
We consider each TP as covered when the planning is such that a certain traffic demand can be guaranteed on both the primary and secondary link. In particular, parameter $D_t$ represents the demand to be guaranteed by the connection with the primary BS. That is, the minimum throughput experienced by TP $t$ when it is connected to its the primary BS. On the secondary link, a fraction $\xi$ of the traffic demand $D_t$ is guaranteed. This represents the throughput available to TP $t$ through the backup link.\par




==> content/figures/README <==
$Id: README 42921 2017-01-10 23:39:44Z karl $
This file is public domain.  (Originally written by Karl Berry, 2009.)

This is the README for the epstopdf script distribution.

Primary distribution point: http://ctan.org/pkg/epstopdf
  (list of mirrors at: http://ctan.org/mirrors)

Home page: http://tug.org/epstopdf/

Run epstopdf --help for the usual list of options, examples, etc.

Mailing list for bugs and discussion: http://lists.tug.org/tex-k
When reporting bugs, please include an input file and command line
options, so the problem can be reproduced.

-------------------------------------------------------------------------
Various test files and a Makefile to exercise them are in the source
repository, which is currently a subdirectory of the texlive Subversion
repo, purely for the developers' convenience:
  http://tug.org/svn/texlive/trunk/Build/source/extra/epstopdf/

The test-binary and test-bin2 files there were supplied by Akira Kakuto and
Reinhard Kotucha.  They contain binary data.  They are public domain.

The test-binhdr* files were supplied by Martin von Gagern, constructed
as follows.  They contain binary junk before the EPS starts.  We also
use these to test different line endings.  These files are public domain.

{ echo -e '%Some\000binary\001comment'; dot -Tps <<< 'digraph{a->b}'; }
  > test-binhdr-lf.eps
tr $'\n' $'\r' <test-binhdr-lf.eps >test-binhdr-cr.ps
unix2dos <test-binhdr-lf.eps >test-binhdr-cr.ps


==> content/figures/epstopdf.1 <==
.TH EPSTOPDF 1 "17 September 2018"
.\" $Id: epstopdf.1 48681 2018-09-16 23:03:58Z karl $
.SH NAME
epstopdf, repstopdf \- convert an EPS file to PDF
.SH SYNOPSIS
\fBepstopdf\fP [\fIoptions\fP] [\fIepsfile\fP [\fIpdffile\fP.pdf]]
.SH DESCRIPTION
By default, \fBepstopdf\fP converts the input PostScript file to PDF,
using Ghostscript.
.PP
\fBEpstopdf\fP transforms the Encapsulated PostScript file \fIepsfile\fP
(or standard input) so that it is guaranteed to start at the 0,0
coordinate, and it sets a page size exactly corresponding to the
BoundingBox.  Thus, the result needs no cropping, and the PDF MediaBox
is correct.  
.PP
By default, the output name is the input name with any extension
replaced by \fB.pdf\fP.  An output name ending with .pdf can also be given
as a second argument on the command line, or the \fB--outfile\fP
(\fB-o\fP) option can be used with any name.
.PP
The output is PDF 1.5 by default; use, e.g.,
.nf
--gsopt=-dCompatibilityLevel=1.7
.fi
to change this. (Until epstopdf 2.28 (released September 2018), the
PDF version was whatever the underlying Ghostscript or other interpreter
produced by default.)
.PP
PJL commands at the start of a file are removed.  DOS EPS binary files
(TN 5002) are supported.
.PP
If the bounding box in the input is incorrect, of course there will
be resulting problems.
.SH OPTIONS
Options may start with either "\fB-\fP" or "\fB--\fP", and may be
unambiguously abbreviated.  It is best to use the full option name in
scripts to avoid possible collisions with new options in the future.
.PP
General script options:
.IP "\fB--help\fP
display help message and exit
.IP "\fB--version\fP
display version information and exit
.IP "\fB--outfile\fP=\fIfile\fP"
write result to \fIfile\fP.  If this option is not given, and
\fB--nogs\fP or \fB--filter\fP is specified, write to standard output;
otherwise, the default is to construct the output file name by replacing
any extension in the input file with `.pdf'.
.IP "\fB--\fP[\fBno\fP]\fBdebug\fP"
write debugging info (default: false).
.IP "\fB--\fP[\fBno\fP]\fBexact\fP"
scan ExactBoundingBox (default: false).
.IP "\fB--\fP[\fBno\fP]\fBfilter\fP"
read standard input and (unless \fB--outfile\fP is given) write standard
output (default: false).
.IP "\fB--\fP[\fBno\fP]\fBgs\fP"
run Ghostscript (default: true).  With \fB--nogs\fP, output (to standard
output by default) the PostScript that would normally be converted; that
is, the input PostScript as modified by \fBepstopdf\fP.
.IP "\fB--\fP[\fBno\fP]\fBhires\fP"
scan HiresBoundingBox (default: false).
.IP "\fB--restricted\fP=\fIval\fP"
turn on restricted mode (default: [true for repstopdf, else false]);
this forbids the use of \fB--gscmd\fP and other options and imposes
restrictions on the input and output file names according to the values
of openin_any and openout_any (see the Web2c manual, http://tug.org/web2c).
.PP
Options for Ghostscript (more info below):
.IP "\fB--gscmd\fP=\fIval\fP"
pipe output to \fIval\fP (default: [\fBgswin32c\fP on Windows, else \fBgs\fP])
.IP "\fB--gsopt\fP=\fIval\fP"
include \fIval\fP as one argument in the gs command (can be repeated).
.IP "\fB--gsopts\fP=\fIval\fP"
split \fIval\fP at whitespace and include each resulting word as an
argument in the gs command (can be repeated).
.IP "\fB--autorotate\fP=\fIval\fP"
set AutoRotatePages (default: None); recognized \fIval\fP choices:
None, All, PageByPage.  For EPS files, PageByPage is equivalent to All.
.IP "\fB--\fP[\fBno\fP]\fBcompress\fP"
use compression in the output (default: true); if turned off, passes
.IR -dUseFlateCompression=false .
.IP "\fB--device\fP=\fIdev\fP"
use -sDEVICE=\fIdev\fP (default: pdfwrite); not allowed in restricted mode.
.IP "\fB--\fP[\fBno\fP]\fBembed\fP"
embed fonts (default: true); passes
.I -dMaxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true.
.IP "\fB--\fP[\fBno\fP]\fBgray\fP"
grayscale output (default: false); passes
.I -sColorConversionStrategy=Gray -dProcessColorModel=/DeviceGray.
.IP "\fB--pdfsettings\fP=\fIval\fP"
use -dPDFSETTINGS=/\fIval\fP (default is `prepress' if \fB--embed\fP,
else empty); recognized \fIval\fP choices: screen, ebook, printer,
prepress, default.
.IP "\fB--\fP[\fBno\fP]\fBquiet\fP"
use -q, a.k.a. -dQUIET (default: false).
.IP "\fB--res\fP=\fIdpi, dpi\fPx\fIdpi\fP"
set image resolution (default: [use gs default]); ignored if
\fB--debug\fP is set.
.IP "\fB--\fP[\fBno\fP]\fBsafer\fP"
use -d(NO)QUIET (default: true).
.PP
In addition to the specific options above, additional options to be used
with gs can be specified with either or both of the two cumulative
options \fB--gsopts\fP and \fB--gsopt.\fP
.PP
\fB--gsopts\fP takes a single string of options, which is split at
whitespace, each resulting word then added to the gs command line
individually.
.PP
\fB--gsopt\fP adds its argument as a single option to the gs command
line.  It can be used multiple times to specify options separately,
and is necessary if an option or its value contains whitespace.
.PP
In restricted mode, options are limited to those with names and values
known to be safe.  Some options taking booleans, integers or fixed
names are allowed, those taking general strings are not.

.SH EXAMPLES
These examples all equivalently convert `test.eps' to `test.pdf':
.nf
epstopdf test.eps
epstopdf test.eps test.pdf
cat test.eps | epstopdf --filter >test.pdf
cat test.eps | epstopdf -f -o=test.pdf
.fi
.PP
Example for using HiResBoundingBox instead of BoundingBox:
.nf
epstopdf --hires test.eps
.fi
.PP
Example for \fBepstopdf\fP's attempt at correcting PostScript:
.nf
$program --nogs test.ps >testcorr.ps
.fi
.PP
In all cases, you can add \fB--debug\fP (\fB-d\fP) to see more about
what \fBepstopdf\fP is doing.
.SH BUGS
The case of "%%BoundingBox: (atend)" when input is not seekable (e.g.,
from a pipe) is not supported.
.PP
Report bugs in the program or this man page to tex-k@tug.org.  When
reporting bugs, please include an input file and the command line
options specified, so the problem can be reproduced.
.SH SEE ALSO
\fBgs\fP(1),
\fBpdfcrop\fP(1).
.PP
The epstopdf LaTeX package, part of the oberdiek bundle, which automates
running this script on the fly under TeX: http://ctan.org/pkg/epstopdf-pkg.
.SH AUTHOR
Originally written by Sebastian Rahtz, for Elsevier Science, with
subsequent contributions from Thomas Esser, Gerben Wierda, Heiko
Oberdiek, and many others.  Currently maintained by Karl Berry.
.PP
Man page originally written by Jim Van Zandt.
.PP
epstopdf home page: http://tug.org/epstopdf.
.PP
You may freely use, modify and/or distribute this man page.


==> content/model.tex <==
begin{maxi!}[3]
  {}{\left\{ \mu \sum_{t \in \T}\frac{\theta_t}{\Theta} + (1-\mu) \sum_{t \in \T} \frac{l_t}{\hat{L}} \right\}}{}{}\label{opt1:obj}
  \addConstraint{y_c^\text{IAB} + y_c^\text{RIS}}{\leq 1}{ \forall c \in \C}\label{opt1:ris_iab_act}
  \addConstraint{y_c^\text{DON}}{\leq y_c^\text{IAB}}{\forall c \in \C}\label{opt1:don_act}
  \addConstraint{\sum_{c \in \C}y_c^\text{DON}}{= 1}{\forall c \in \C}\label{opt1:only_1_don}
  \addConstraint{\sum_{c \in \C}\left( P^\text{IAB}y_c^\text{IAB} + P^\text{RIS}y_c^\text{RIS}\right)}{\leq B}{}\label{opt:budget}
  \addConstraint{x_{t,c,r}}{\leq \Lambda_{t,c,r}^\text{SRC}\left(y_c^\text{IAB} \land y_r^\text{RIS}\right)}{\forall t \in \T, c,r \in \C}\label{opt:link_act_1}
  \addConstraint{z_{c,d}}{\leq \Lambda_{c,d}^\text{BH}\left(y_c^\text{IAB} \land y_d^\text{IAB}\right)}{\forall c,d \in \C}\label{opt:link_act_2}
  \addConstraint{\sum_{c,r \in \C}x_{t,c,r}}{=1}{\forall t \in \T}\label{opt:only_1_src}
  \addConstraint{w_{c} + \sum_{d \in C} (f_{d,c} - f_{c,d})-\sum_{\substack{t \in T\\r \in \C}} D x_{t,c,r}}{=0}{\forall c \in \C}\label{opt:flow_balance}
  \addConstraint{ w_c}{ \leq U^{WRD} y_c^{\text{DON}}}{\forall c \in \C}\label{opt:core_flow}
  \addConstraint{f_{c,d}}{\leq z_{c,d}U_{c,d}}{\forall c,d \in \C}\label{opt:bh_capacity}
  \addConstraint{D x_{t,c,r}}{\leq V_{t,c,r}^{\text{DIR}}}{\forall t \in \T, c,r \in \C}\label{opt:dir_acc_cap}
  \addConstraint{\xi D x_{t,c,r}}{\leq V_{t,c,r}^{\text{REF}}}{\forall t \in \T, c,r \in \C}\label{opt:ref_acc_cap}
  \addConstraint{t_c^{\text{TX}}} {= \sum_{d \in \C} \frac{f_{c,d}}{U_{c,d}} + \sum_{t \in T, r \in \C}\frac{D_t x_{t,c,r}} {V^{DIR}_{t,c,r}}}{\forall c \in \C}\label{opt:tx_time}
  \addConstraint{t_{c}^{\text{RX}}}{ = \sum_{d \in \C} \frac{f_{d,c}} {U_{d,c}}}{\forall c \in \C}\label{opt:rx_time}
  \addConstraint{t_c^{\text{TX}} + t_c^{\text{RX}}} {\leq y_c^{\text{IAB}}}{\forall c \in \C}\label{opt:hd}
  \addConstraint{\sum_{d \in C}z_{d,c}}{ \leq 1 - y_c^{\text{DON}}}{\forall c \in \C}\label{opt:span_tree_1}
  %\addConstraint{z_{c,d}+z_{d,c}}{\leq 1}{\forall c,d \in \C}
  \addConstraint{\tau_{t,c,r}}{ \leq x_{t,c,r}}{\forall t \in \T, c,r \in \C}\label{opt:tdm_act}
  \addConstraint{\sum_{t \in T, c \in C} \tau_{t,c,r}} {\leq y_r^{\text{RIS}}}{\forall r \in \C}\label{opt:tdm_inst}
  \addConstraint{\tau_{t,c,r}}{ \geq \frac{D} {V^{DIR}_{t,c,r}} -(1 - x_{t,c,r})}{\forall t \in \T, c,r \in \C}\label{opt:ris_tdm}
  \addConstraint{\phi_r}{\geq \Phi^{\text{A}}_{r,t} - D/2 - 2\pi(\neg x_{t,d,r})}{\forall t \in \T, d,r \in \C}\label{opti2:or1}
  \addConstraint{\phi_r}{\leq \Phi^{\text{A}}_{r,t} + D/2 + 2\pi(\neg x_{t,d,r})}{\forall t \in \T, d,r \in \C}\label{opti2:or2}
  \addConstraint{\phi_r}{\geq \Phi^{\text{B}}_{r,d} - D/2 - 2\pi(\neg x_{t,d,r})}{\forall t \in \T, d,r \in \C}\label{opti2:or3}
  \addConstraint{\phi_r}{\leq \Phi^{\text{B}}_{r,d} + D/2 + 2\pi(\neg x_{t,d,r})}{\forall t \in \T, d,r \in \C}\label{opti2:or4}
  \addConstraint{\theta_{t}}{ \leq \Theta_{t,c,r} + 2 \pi(1-x_{t,c,r})}{\forall t \in \T, c,r \in\C}\label{opt:ang_sep}
  \addConstraint{\lambda_t} {\geq \frac{1}{2}\sum_{c,r \in \C}x_{t,c,r} (L_{t,r} + L_{t,d})}{\forall t \in \T}\label{opt:lin_len}
\end{maxi!}

